Constraint-based Task Specification and Trajectory Optimization for Sequential Manipulation

To economically deploy robotic manipulators the programming and execution of robot motions must be swift. To this end, we propose a novel, constraint-based method to intuitively specify sequential manipulation tasks and to compute time-optimal robot motions for such a task specification. Our approach follows the ideas of constraint-based task specification by aiming for a minimal and object-centric task description that is largely independent of the underlying robot kinematics. We transform this task description into a non-linear optimization problem. By solving this problem we obtain a (locally) time-optimal robot motion, not just for a single motion, but for an entire manipulation sequence. We demonstrate the capabilities of our approach in a series of experiments involving five distinct robot models, including a highly redundant mobile manipulator.

==> image.tex <==
\begin{tikzpicture}[   scale=1.25]


	% box corner coordinates
	\coordinate (ctr) at (1.0, 1.0);
	\coordinate (cbr) at (1.0, -1.0);
	\coordinate (ctl) at (-1.0, 1.0);
	\coordinate (cbl) at (-1.0, -1.0);
	
	% box center positions
	\coordinate (s_one) at (0.0, 0.0);
	\coordinate (s_two) at (-1.2, -2.4);
	\coordinate (s_three) at (1.2, -2.4);
	\coordinate (s_four) at (-2.4, -4.8);
	\coordinate (s_five) at (0.0, -4.8);
	\coordinate (s_six) at (2.4, -4.8);

	% boxes
	\draw [draw=black, fill=black, fill opacity=0.3] plot coordinates {($(s_one)+(ctr)$) ($(s_one)+(cbr)$) ($(s_one)+(cbl)$) ($(s_one)+(ctl)$) ($(s_one)+(ctr)$)};
	%\draw [pattern=north east lines, pattern color=black] plot coordinates {($(s_one)+(ctr)$) ($(s_one)+(cbr)$) ($(s_one)+(cbl)$) ($(s_one)+(ctl)$) ($(s_one)+(ctr)$)};	
	
	\draw [draw=black, fill=black, fill opacity=0.3] plot coordinates {($(s_two)+(ctr)$) ($(s_two)+(cbr)$) ($(s_two)+(cbl)$) ($(s_two)+(ctl)$) ($(s_two)+(ctr)$)};
	\draw [draw=black, fill=black, fill opacity=0.3] plot coordinates {($(s_three)+(ctr)$) ($(s_three)+(cbr)$) ($(s_three)+(cbl)$) ($(s_three)+(ctl)$) ($(s_three)+(ctr)$)};
	\draw [draw=black, fill=black, fill opacity=0.3] plot coordinates {($(s_four)+(ctr)$) ($(s_four)+(cbr)$) ($(s_four)+(cbl)$) ($(s_four)+(ctl)$) ($(s_four)+(ctr)$)};
	\draw [draw=black, fill=black, fill opacity=0.3] plot coordinates {($(s_five)+(ctr)$) ($(s_five)+(cbr)$) ($(s_five)+(cbl)$) ($(s_five)+(ctl)$) ($(s_five)+(ctr)$)};
	
	\draw [draw=black, fill=black, fill opacity=0.3] plot coordinates {($(s_six)+(ctr)$) ($(s_six)+(cbr)$) ($(s_six)+(cbl)$) ($(s_six)+(ctl)$) ($(s_six)+(ctr)$)};
	%\draw [pattern=north east lines, pattern color=black] plot coordinates {($(s_six)+(ctr)$) ($(s_six)+(cbr)$) ($(s_six)+(cbl)$) ($(s_six)+(ctl)$) ($(s_six)+(ctr)$)};
	


	\coordinate (one_a) at (0.8, -0.8);
	\coordinate (one_b) at (0.8, 0.8);
	\coordinate (one_c) at (0.0, 0.9);
	\coordinate (one_d) at (-0.5, 0.5);
	\coordinate (one_e) at (-0.8, 0.0);
	\coordinate (one_f) at (-0.5, -0.8);
	\coordinate (one_g) at (0.1, -0.4);
	\coordinate (one_h) at (0.5, -0.8);
	
	\draw [draw=black, fill=white, fill opacity=1.0] plot [smooth cycle] coordinates {($(s_one)+(one_a)$) ($(s_one)+(one_b)$) ($(s_one)+(one_c)$) ($(s_one)+(one_d)$) ($(s_one)+(one_e)$) ($(s_one)+(one_f)$) ($(s_one)+(one_g)$) ($(s_one)+(one_h)$)};
	
	\coordinate (two_a) at (0.8, 0.0);
	\coordinate (two_b) at (0.85, 0.85);
	\coordinate (two_c) at (0.2, 0.8);
	\coordinate (two_d) at (-0.5, 0.2);
	\coordinate (two_e) at (-0.8, 0.0);
	\coordinate (two_f) at (-0.5, -0.8);
	\coordinate (two_g) at (0.0, -0.8);
	\coordinate (two_h) at (0.5, -0.5);
	
	\draw [draw=black, fill=white, fill opacity=1.0] plot [smooth cycle] coordinates {($(s_two)+(two_a)$) ($(s_two)+(two_b)$) ($(s_two)+(two_c)$) ($(s_two)+(two_d)$) ($(s_two)+(two_e)$) ($(s_two)+(two_f)$) ($(s_two)+(two_g)$) ($(s_two)+(two_h)$)};
	
	\coordinate (three_a) at (0.8, 0.0);
	\coordinate (three_b) at (0.5, 0.5);
	\coordinate (three_c) at (0.0, 0.4);
	\coordinate (three_d) at (-0.75, 0.75);
	\coordinate (three_e) at (-0.6, 0.0);
	\coordinate (three_f) at (-0.7, -0.8);
	\coordinate (three_g) at (0.0, -0.6);
	\coordinate (three_h) at (0.7, -0.8);
	
	\draw [draw=black, fill=white, fill opacity=1.0] plot [smooth cycle] coordinates {($(s_three)+(three_a)$) ($(s_three)+(three_b)$) ($(s_three)+(three_c)$) ($(s_three)+(three_d)$) ($(s_three)+(three_e)$) ($(s_three)+(three_f)$) ($(s_three)+(three_g)$) ($(s_three)+(three_h)$)};
	
	\coordinate (four_a) at (0.6, 0.9);
	\coordinate (four_b) at (0.9, 0.6);
	\coordinate (four_c) at (0.6, 0.3);
	\coordinate (four_d) at (0.0, 0.0);
	\coordinate (four_e) at (0.0, -0.1);
	\coordinate (four_f) at (0.7, -0.2);
	\coordinate (four_g) at (0.8, -0.5);
	\coordinate (four_h) at (0.5, -0.95);
	\coordinate (four_i) at (-0.8, -0.7);
	\coordinate (four_j) at (-0.5, 0.7);
	
	\draw [draw=black, fill=white, fill opacity=1.0] plot [smooth cycle] coordinates {($(s_four)+(four_a)$) ($(s_four)+(four_b)$) ($(s_four)+(four_c)$) ($(s_four)+(four_d)$) ($(s_four)+(four_e)$) ($(s_four)+(four_f)$) ($(s_four)+(four_g)$) ($(s_four)+(four_h)$) ($(s_four)+(four_i)$) ($(s_four)+(four_j)$)};
	
	
	\coordinate (goal_a) at (0.6, -0.3);
	\coordinate (goal_b) at (0.7, -0.5);
	\coordinate (goal_c) at (0.4, -0.7);
	\coordinate (goal_d) at (-0.0, -0.5);
	\coordinate (goal_e) at (0.2, -0.2);
	
	\draw [pattern=north east lines, pattern color=orange] plot [smooth cycle] coordinates {($(s_four)+(goal_a)$) ($(s_four)+(goal_b)$) ($(s_four)+(goal_c)$) ($(s_four)+(goal_d)$) ($(s_four)+(goal_e)$)};
	
	\coordinate (five_a) at (0.1, 0.6);
	\coordinate (five_b) at (0.4, -0.2);
	\coordinate (five_c) at (0.8, 0.1);
	\coordinate (five_d) at (0.7, 0.8);
	
	\coordinate (five_e) at (-0.4, 0.8);
	\coordinate (five_f) at (-0.1, -0.3);
	\coordinate (five_g) at (0.6, -0.6);
	\coordinate (five_h) at (0.3, -0.8);
	\coordinate (five_i) at (-0.5, -0.7);
	\coordinate (five_j) at (-0.8, 0.4);
	
	\draw [draw=black, fill=white, fill opacity=1.0] plot [smooth cycle] coordinates {($(s_five)+(five_a)$) ($(s_five)+(five_b)$) ($(s_five)+(five_c)$) ($(s_five)+(five_d)$)};
	
	\draw [draw=black, fill=white, fill opacity=1.0] plot [smooth cycle] coordinates {($(s_five)+(five_e)$) ($(s_five)+(five_f)$) ($(s_five)+(five_g)$) ($(s_five)+(five_h)$) ($(s_five)+(five_i)$) ($(s_five)+(five_j)$)};
	
	\coordinate (goal2_a) at (-0.4, 0.4);
	\coordinate (goal2_b) at (-0.2, -0.3);
	\coordinate (goal2_c) at (-0.5, -0.2);
	\coordinate (goal2_d) at (-0.6, 0.1);
	
	\draw [pattern=north east lines, pattern color=orange] plot [smooth cycle] coordinates {($(s_five)+(goal2_a)$) ($(s_five)+(goal2_b)$) ($(s_five)+(goal2_c)$) ($(s_five)+(goal2_d)$)};	
	
	
	
	
	\coordinate (six_a) at (0.6, 0.7);
	\coordinate (six_b) at (0.8, -0.7);
	\coordinate (six_c) at (0.2, -0.9);
	\coordinate (six_d) at (-0.5, -0.8);
	\coordinate (six_e) at (-0.8, 0.1);
	\coordinate (six_f) at (-0.4, 0.8);
	
	\coordinate (six_g) at (0.4, -0.1);
	\coordinate (six_h) at (-0.2, 0.4);
	\coordinate (six_i) at (-0.3, -0.2);
	
	\draw [draw=black, fill=white, fill opacity=1.0] plot [smooth cycle] coordinates {($(s_six)+(six_a)$) ($(s_six)+(six_b)$) ($(s_six)+(six_c)$) ($(s_six)+(six_d)$) ($(s_six)+(six_e)$) ($(s_six)+(six_f)$)};
	
	\draw [draw=black, fill=black, fill opacity=0.3] plot [smooth cycle] coordinates {($(s_six)+(six_g)$) ($(s_six)+(six_h)$) ($(s_six)+(six_i)$)};




	
	\coordinate (pstart) at (0.7,0.7);	
	
	\coordinate (v11) at (0.3,0.65);		
	\coordinate (p11) at (0.0,0.5);	
	
	\coordinate (v12) at (-0.2,0.15);		
	\coordinate (p12) at (0.1,-0.2);	
	
	\coordinate (v13) at (0.3,-0.3);		
	\coordinate (p13) at (0.4,0.0);	
	
	\coordinate (v14) at (-0.4,0.0);		
	\coordinate (p14) at (-0.5, -0.6);	% Transition
	
	\coordinate (v15) at (0.2, -0.3);		
	\coordinate (p15) at (0.7, -0.6);	% Transition
	
	
	\draw [draw=black] plot [smooth] coordinates {($(s_one)+(pstart)$) ($(s_one)+(v11)$) ($(s_one)+(p11)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_one)+(p11)$) ($(s_one)+(v12)$) ($(s_one)+(p12)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_one)+(p12)$) ($(s_one)+(v13)$) ($(s_one)+(p13)$)};
	
	
	\draw [draw=black, line width=0.5mm] plot [smooth] coordinates {($(s_one)+(p11)$) ($(s_one)+(v14)$) ($(s_one)+(p14)$)}; %Transition action
	\draw [draw=blue, line width=0.8mm, opacity=0.7] plot [smooth] coordinates {($(s_one)+(p14)+(-0.15, 0.2)$) ($(s_one)+(p14)$) ($(s_one)+(p14)+(0.2, 0.05)$)}; % Transition Area
	
	\draw [draw=black, line width=0.5mm] plot [smooth] coordinates {($(s_one)+(p12)$) ($(s_one)+(v15)$) ($(s_one)+(p15)$)}; %Transition action
	\draw [draw=blue, line width=0.8mm, opacity=0.7] plot [smooth] coordinates {($(s_one)+(p15)+(-0.1, -0.1)$) ($(s_one)+(p15)$) ($(s_one)+(p15)+(0.05, 0.15)$)}; % Transition Area
	
	\draw [fill=black, fill opacity=1] ($(s_one)+(pstart)$) circle [radius=0.06];
	\draw [fill=white, fill opacity=1] ($(s_one)+(pstart)$) circle [radius=0.04];
	
	\draw [fill=black, fill opacity=1] ($(s_one)+(p11)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_one)+(p12)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_one)+(p13)$) circle [radius=0.04];
	
	\draw [fill=black, fill opacity=1] ($(s_one)+(p14)$) circle [radius=0.04]; % Transition
	\draw [fill=black, fill opacity=1] ($(s_one)+(p15)$) circle [radius=0.04]; % Transition
	


	\coordinate (p21) at (0.7,0.7);	
	
	\coordinate (v22) at (0.65, 0.45);	
	\coordinate (p22) at (0.75, 0.2);	
	
	\coordinate (v23) at (0.55, 0.55);	
	\coordinate (p23) at (0.4, 0.5);	
	
	\coordinate (v24) at (0.2, 0.45);	
	\coordinate (p24) at (0.0, 0.5);	
	
	\coordinate (v25) at (0.2, 0.2);	
	\coordinate (p25) at (0.25, -0.05);	
	
	\coordinate (v26) at (0.4, -0.15);	
	\coordinate (p26) at (0.5, -0.1);	
	
	\coordinate (v27) at (0.2, -0.4);	
	\coordinate (p27) at (-0.2, -0.5);	
	
	\coordinate (v28) at (-0.35, -0.5);	
	\coordinate (p28) at (-0.4, -0.6);	
			
	\draw [draw=black, dashed, line width=0.6mm] plot [smooth] coordinates {($(s_one)+(p14)$) ($(s_two)+(p21)$)};	
	%\draw [draw=blue, line width=0.8mm, opacity=0.7] plot [smooth] coordinates {($(s_two)+(p21)+(-0.25, -0.05)$) ($(s_two)+(p21)$) ($(s_two)+(p21)+(0.05, -0.2)$)}; % Transition Area
	
	\draw [draw=black] plot [smooth] coordinates {($(s_two)+(p21)$) ($(s_two)+(v22)$) ($(s_two)+(p22)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_two)+(p21)$) ($(s_two)+(v23)$) ($(s_two)+(p23)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_two)+(p23)$) ($(s_two)+(v24)$) ($(s_two)+(p24)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_two)+(p23)$) ($(s_two)+(v25)$) ($(s_two)+(p25)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_two)+(p25)$) ($(s_two)+(v26)$) ($(s_two)+(p26)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_two)+(p25)$) ($(s_two)+(v27)$) ($(s_two)+(p27)$)};	
	
	\draw [draw=black, line width=0.5mm] plot [smooth] coordinates {($(s_two)+(p27)$) ($(s_two)+(v28)$) ($(s_two)+(p28)$)}; %Transition action
	\draw [draw=blue, line width=0.8mm, opacity=0.7] plot [smooth] coordinates {($(s_two)+(p28)+(-0.15, 0.2)$) ($(s_two)+(p28)$) ($(s_two)+(p28)+(0.2, -0.05)$)}; % Transition Area
	
	\draw [fill=black, fill opacity=1] ($(s_two)+(p21)$) circle [radius=0.04]; % Transition
	\draw [fill=black, fill opacity=1] ($(s_two)+(p22)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_two)+(p23)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_two)+(p24)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_two)+(p25)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_two)+(p26)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_two)+(p27)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_two)+(p28)$) circle [radius=0.04]; % Transition
	
	
	
	
	\coordinate (p31) at (0.4,0.3);	
	
	\coordinate (v32) at (0.2, 0.0);	
	\coordinate (p32) at (-0.1, -0.1);	
	
	\coordinate (v33) at (-0.25, 0.05);	
	\coordinate (p33) at (-0.3, 0.3);	
	
	\coordinate (v34) at (-0.4, -0.2);	
	\coordinate (p34) at (-0.5, -0.6);	
	
	\coordinate (p35) at (0.6, -0.6);	
				
		
	\draw [draw=black, dashed, line width=0.6mm] plot [smooth] coordinates {($(s_one)+(p15)$) ($(s_three)+(p31)$)};	
	%\draw [draw=blue, line width=0.8mm, opacity=0.7] plot [smooth] coordinates {($(s_three)+(p31)+(-0.25, -0.05)$) ($(s_three)+(p31)$) ($(s_three)+(p31)+(0.15, -0.02)$)}; % Transition Area
	
	\draw [draw=black] plot [smooth] coordinates {($(s_three)+(p31)$) ($(s_three)+(v32)$) ($(s_three)+(p32)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_three)+(p32)$) ($(s_three)+(v33)$) ($(s_three)+(p33)$)};

	
	\draw [draw=black, line width=0.5mm] plot [smooth] coordinates {($(s_three)+(p32)$) ($(s_three)+(v34)$) ($(s_three)+(p34)$)}; %Transition action
	\draw [draw=blue, line width=0.8mm, opacity=0.7] plot [smooth] coordinates {($(s_three)+(p34)+(-0.15, 0.2)$) ($(s_three)+(p34)$) ($(s_three)+(p34)+(0.2, -0.05)$)}; % Transition Area
	
	\draw [draw=black, line width=0.5mm] plot [smooth] coordinates {($(s_three)+(p31)$) ($(s_three)+(p35)$)}; %Transition action
	\draw [draw=blue, line width=0.8mm, opacity=0.7] plot [smooth] coordinates {($(s_three)+(p35)+(-0.15, 0.0)$) ($(s_three)+(p35)$) ($(s_three)+(p35)+(0.15, 0.05)$)}; % Transition Area
	
	\draw [fill=black, fill opacity=1] ($(s_three)+(p31)$) circle [radius=0.04]; % Transition
	\draw [fill=black, fill opacity=1] ($(s_three)+(p32)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_three)+(p33)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_three)+(p34)$) circle [radius=0.04]; % Transition
	\draw [fill=black, fill opacity=1] ($(s_three)+(p35)$) circle [radius=0.04]; % Transition

	
	\coordinate (p41) at (0.6,0.7);	
	
	\coordinate (v42) at (0.45, 0.4);	
	\coordinate (p42) at (0.0, 0.3);	
	
	\coordinate (v43) at (-0.3, 0.45);	
	\coordinate (p43) at (-0.1, 0.6);	
	
	\coordinate (v44) at (-0.6, 0.0);	
	\coordinate (p44) at (-0.3, -0.4);	
	
	\coordinate (v45) at (0.0, -0.55);	
	\coordinate (p45) at (0.5, -0.4);	
	
	\draw [draw=black, dashed, line width=0.6mm] plot [smooth] coordinates {($(s_two)+(p28)$) ($(s_four)+(p41)$)};	
	%\draw [draw=blue, line width=0.8mm, opacity=0.7] plot [smooth] coordinates {($(s_four)+(p41)+(-0.15, 0.05)$) ($(s_four)+(p41)$) ($(s_four)+(p41)+(0.2, -0.1)$)}; % Transition Area
	
	\draw [draw=black] plot [smooth] coordinates {($(s_four)+(p41)$) ($(s_four)+(v42)$) ($(s_four)+(p42)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_four)+(p42)$) ($(s_four)+(v43)$) ($(s_four)+(p43)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_four)+(p42)$) ($(s_four)+(v44)$) ($(s_four)+(p44)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_four)+(p44)$) ($(s_four)+(v45)$) ($(s_four)+(p45)$)};
	
	\draw [fill=black, fill opacity=1] ($(s_four)+(p41)$) circle [radius=0.04]; % Transition
	\draw [fill=black, fill opacity=1] ($(s_four)+(p42)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_four)+(p43)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_four)+(p44)$) circle [radius=0.04]; 
	\draw [fill=black, fill opacity=1] ($(s_four)+(p45)$) circle [radius=0.04]; % Goal
	
	
	
	\coordinate (p51) at (0.5,0.6);	
	
	\coordinate (v52) at (0.47, 0.3);	
	\coordinate (p52) at (0.4, 0.1);	
	
	\coordinate (v53) at (0.55, 0.35);	
	\coordinate (p53) at (0.7, 0.2);
	
	\draw [draw=black, dashed, line width=0.6mm] plot [smooth] coordinates {($(s_three)+(p34)$) ($(s_five)+(p51)$)};	
	%\draw [draw=blue, line width=0.8mm, opacity=0.7] plot [smooth] coordinates {($(s_five)+(p51)+(-0.1, -0.05)$) ($(s_five)+(p51)$) ($(s_five)+(p51)+(0.1, 0.0)$)}; % Transition Area
	
	\draw [draw=black] plot [smooth] coordinates {($(s_five)+(p51)$) ($(s_five)+(v52)$) ($(s_five)+(p52)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_five)+(p51)$) ($(s_five)+(v53)$) ($(s_five)+(p53)$)};
	
	\draw [fill=black, fill opacity=1] ($(s_five)+(p51)$) circle [radius=0.04]; % Transition
	\draw [fill=black, fill opacity=1] ($(s_five)+(p52)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_five)+(p53)$) circle [radius=0.04];
	
	\coordinate (p61) at (0.6,-0.6);	
	
	\coordinate (v62) at (0.6, -0.3);	
	\coordinate (p62) at (0.5, -0.1);	
	
	\coordinate (v63) at (0.0, -0.65);	
	\coordinate (p63) at (-0.3, -0.4);
	
	\coordinate (v64) at (-0.5, 0.0);	
	\coordinate (p64) at (-0.4, 0.3);	
	
	\coordinate (v65) at (-0.15, 0.5);	
	\coordinate (p65) at (0.2, 0.5);
	
	
	\draw [draw=black, dashed, line width=0.6mm] plot [smooth] coordinates {($(s_three)+(p35)$) ($(s_six)+(p61)$)};
	
	\draw [draw=black] plot [smooth] coordinates {($(s_six)+(p61)$) ($(s_six)+(v62)$) ($(s_six)+(p62)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_six)+(p61)$) ($(s_six)+(v63)$) ($(s_six)+(p63)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_six)+(p63)$) ($(s_six)+(v64)$) ($(s_six)+(p64)$)};
	\draw [draw=black] plot [smooth] coordinates {($(s_six)+(p64)$) ($(s_six)+(v65)$) ($(s_six)+(p65)$)};
	
	
	\draw [fill=black, fill opacity=1] ($(s_six)+(p61)$) circle [radius=0.04]; % Transition
	\draw [fill=black, fill opacity=1] ($(s_six)+(p62)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_six)+(p63)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_six)+(p64)$) circle [radius=0.04];
	\draw [fill=black, fill opacity=1] ($(s_six)+(p65)$) circle [radius=0.04];
	
	
	
\node[text width=2cm, align=center] at ($(s_one)+(0.6, 0.5)$) 
{\small $c_{\text{start}}$\normalsize};
	
\node[text width=2cm, align=center] at ($(s_one)+(0.0, 1.15)$) 
{\small $\sigma_{\text{start}}$\normalsize};	
	
\node[text width=0.3cm, align=center] at ($(s_two)+(-0.8, 1.15)$) 
{\small $\sigma_1$\normalsize};	

\node[text width=0.3cm, align=center] at ($(s_three)+(0.8, 1.15)$) 
{\small $\sigma_2$\normalsize};	

\node[text width=0.3cm, align=center] at ($(s_four)+(-0.8, 1.15)$) 
{\small $\sigma_3$\normalsize};	

\node[text width=2cm, align=center] at ($(s_four)+(0.2, -0.8)$) 
{\small $\mathcal{X}_{\text{goal}}$\normalsize};	

\node[text width=2cm, align=center] at ($(s_five)+(0.0, 1.15)$) 
{\small $\sigma_4$\normalsize};	

\node[text width=2cm, align=center] at ($(s_five)+(-0.25, -0.5)$) 
{\small $\mathcal{X}_{\text{goal}}$\normalsize};

\node[text width=0.3cm, align=center] at ($(s_six)+(0.8, 1.15)$) 
{\small $\sigma_5$\normalsize};		
	
	
	
	

	%\coordinate (p2) at (0.2,0.8);	
	%\draw [] ($(o2)+(p1)$) -- ($(o2)+(p2)$);
	%\draw [] ($(o3)+(p1)$) -- ($(o3)+(p2)$);
	%\draw [] ($(o2)+(p2)$) -- ($(o2)+(t1)$);
	%\draw [fill=black, fill opacity=1] ($(o2)+(p2)$) circle [radius=0.04];
	%\draw [fill=black, fill opacity=1] ($(o3)+(p2)$) circle [radius=0.04];




	%\coordinate (cfree) at (1.8,-0.6);

	%\coordinate (c1) at (4,1);
	%\draw [draw=black, fill=green, fill opacity=0.2] plot [smooth cycle] coordinates {($(c1)+(1,0)$) ($(c1)+(1,2)$) ($(c1)+(0.2,3.8)$) ($(c1)+(2,4)$) ($(c1)+(3,2)$) ($(c1)+(2,0)$) };
	%\draw [draw=black] ($(c1)+(0,0)$) -- ($(c1)+(0,4)$)  -- ($(c1)+(2,4)$) -- ($(c1)+(2,0)$) ;	
	 
	%transition area
	%\draw [draw=black, fill=blue, fill opacity=0.2] plot [smooth cycle] coordinates {($(c1)+(1.4,0.4)$) ($(c1)+(1.4,0.8)$) ($(c1)+(1.9,0.8)$) ($(c1)+(1.9,0.4)$) };
	%\draw [pattern=north east lines, pattern color=blue] plot [smooth cycle] coordinates {($(c1)+(1.4,0.4)$) ($(c1)+(1.4,0.8)$) ($(c1)+(1.9,0.8)$) ($(c1)+(1.9,0.4)$) };	
	
	%goal area
	%\draw [draw=black, fill=red, fill opacity=0.3] plot [smooth cycle] coordinates {($(c1)+(1.2,2.4)$) ($(c1)+(1.0,3.8)$) ($(c1)+(2.2,3.4)$) ($(c1)+(1.9,2.4)$) };	
	%\node[text width=2cm, align=center] at ($(c1)+(1.7,3.2)$) 
	%{\small $\mathcal{C}_\text{goal}$\normalsize};	
	
	%\node[text width=2cm, align=center] at ($(c1)+(cfree)$) 
	%{$\mathcal{C}_{\text{free},\sigma_{S2}}$};		
			  
	%\coordinate (c1) at (2,0.5);
	%cfree
	%\draw [draw=black, fill=green, fill opacity=0.2] plot [smooth cycle] coordinates {($(c1)+(0,0.5)$) ($(c1)+(-0.5,2)$) ($(c1)+(0,4)$) ($(c1)+(2,4)$) ($(c1)+(2.5,2)$) ($(c1)+(2,0)$) ($(c1)+(1,0.5)$)};
	%hole in cfree
	%\draw [draw=black, fill=white, fill opacity=1] plot [smooth cycle] coordinates {($(c1)+(0.3,1.8)$) ($(c1)+(0.5,3)$) ($(c1)+(1.5,2.5)$) ($(c1)+(1.5,1.5)$) };
	%transition area 1
	%\draw [draw=black, fill=blue, fill opacity=0.2] plot [smooth cycle] coordinates {($(c1)+(1.4,0.4)$) ($(c1)+(1.4,0.8)$) ($(c1)+(1.9,0.8)$) ($(c1)+(1.9,0.4)$) };	
	%\draw [pattern=north east lines, pattern color=blue] plot [smooth cycle] coordinates {($(c1)+(1.4,0.4)$) ($(c1)+(1.4,0.8)$) ($(c1)+(1.9,0.8)$) ($(c1)+(1.9,0.4)$) };			  
	%transition area 2
	%\draw [draw=black, fill=blue, fill opacity=0.2] plot [smooth cycle] coordinates {($(c1)+(0.6,3.6)$) ($(c1)+(0.4,3.8)$) ($(c1)+(0.9,4)$) ($(c1)+(0.9,3.4)$) };
	%\draw [pattern=north east lines, pattern color=blue] plot [smooth cycle] coordinates {($(c1)+(0.6,3.6)$) ($(c1)+(0.4,3.8)$) ($(c1)+(0.9,4)$) ($(c1)+(0.9,3.4)$) };				  
	
	
\end{tikzpicture}
